Links of Second Smallest Knot Floer Homology

We prove that the rank of knot Floer homology detects the Hopf links, and generalize this result further to classify the links of the second smallest knot Floer homology. We also prove a knot Floer homology analog of arXiv:1910.04246v1 [math.GT] and give a partial answer to when the equality holds in the rank inequality between the knot Floer homology of a link and its sublinks.

==> BS.tex <==
\section{Homological action in bordered-sutured manifolds}

$(\Sigma,\overline{\alpha}, \beta, \mathbf{z})$: BS Heegaard diagram\\
$\mathcal{Z}$: arc diagram induced from $\alpha^a$\\
$F=F(\mathcal{Z})$: sutured surface induced from $\mathcal{Z}$ (the bordered part of $\partial Y$)\\

Homological linear independancy condition:
\begin{align*}
    \pi_0(\Sigma\setminus \alpha) \twoheadleftarrow |\mathbf{z}| \twoheadrightarrow \pi_0(\Sigma \setminus \beta) 
\end{align*}
Corollary of this:
\begin{align*}
    \pi_0(\partial \Sigma \setminus \mathcal{Z})\twoheadrightarrow \pi_0(\partial Y\setminus F)
\end{align*}
Hence $H_1(\Sigma, \partial \Sigma \setminus \mathcal{Z})\twoheadrightarrow H_1(Y, \partial Y\setminus F)$ holds for such a BS Heegaard diagram.\\
$\zeta\in H_1(Y,\partial Y\setminus F)$ can be represented by a relative 1-cycle $\omega$ in $(\Sigma, \partial \Sigma \setminus \mathcal{Z})$.
\begin{align*}
    A_\omega (\mathbf{x})=\sum \# \widehat{\mathcal{M}}(\phi)t^{\omega\cdot \partial_\alpha \phi}\mathbf{y}
\end{align*}
As in \cite[Lemma 2.4]{niHomologicalActionsSutured2014}, this defines a $H_1(Y,\partial Y\setminus F)$ action on $\underline{\widehat{CFD}}$ and $\underline{\widehat{CFA}}$.\\
In terms of twisted coefficient-homological action analogy, as $\pi_2(\mathbf{x},\mathbf{x})\cong H_2(Y,F)$ and its Poincare-Lefschetz dual is $H_1(Y,\partial Y\setminus F)$, the action of the group $H_1(Y,\partial Y\setminus F)$ is natural to expect.\\

